Instance-Level Safety-Aware Fidelity of Synthetic Data and Its Calibration

Modeling and calibrating the fidelity of synthetic data is paramount in shaping the future of safe and reliable self-driving technology by offering a cost-effective and scalable alternative to real-world data collection. We focus on its role in safety-critical applications, introducing four types of instance-level fidelity that go beyond mere visual input characteristics. The aim is to ensure that applying testing on synthetic data can reveal real-world safety issues, and the absence of safety-critical issues when testing under synthetic data can provide a strong safety guarantee in real-world behavior. We suggest an optimization method to refine the synthetic data generator, reducing fidelity gaps identified by deep learning components. Experiments show this tuning enhances the correlation between safety-critical errors in synthetic and real data.

==> macro.tex <==
\newcommand{\commentout}[1]{}

\newcommand{\dnnfunction}{\phi}
\newcommand{\rnnfunction}{\psi}
\newcommand{\covered}[3]{{#1}_{#2}#3}
\newcommand{\valuefunction}{g}
\newcommand{\featureactivation}{a}
\newcommand{\neuronpair}{\alpha}
\newcommand{\feature}{\psi}
\newcommand{\features}{\Psi}
\newcommand{\neuronpairs}{\mathsf{O}}
\newcommand{\testsuite}{\mathcal{T}}
\newcommand{\distance}[2]{ ||#1||_{#2}}
\newcommand{\powerset}[1]{{\cal P}(#1)}
\newcommand{\real}{\mathbb{R}}

\newcommand{\sequence}[1]{\mathtt{#1}}
\newcommand{\metric}{M}
\newcommand{\network}{{\cal N}}
\newcommand{\requirement}{{\cal R}}
\newcommand{\assertmethod}{{\cal A}}

\newcommand{\testRNN}{\textbf{testRNN}}

\newcommand{\param}[1]{\texttt{#1}}
\newcommand{\num}[2]{$#1$$,$$#2$}

\newcommand{\context}{{\cal C}}
\newcommand{\contexts}{{\tt C}}
\newcommand{\model}{{\cal M}}
\newcommand{\trainingAlgorithm}{{\cal A}}
\newcommand{\networks}{{\tt N}}
\newcommand{\inputdomain}{{\tt X}}
\newcommand{\outputdomain}{{\tt Y}}

\newcommand{\dist}{{\cal D}}

\newcommand{\explanations}{{\cal{E}}}
\newcommand{\explain}{{\tt expl}}

\newcommand{\dimension}{{\tt V}}


\newcommand{\varX}{{\cal X}}
\newcommand{\varY}{{\cal Y}}
\newcommand{\varZ}{{\cal Z}}


